Beyond End-to-End: Dynamic Chain Optimization for Private LLM Adaptation on the Edge

Federated fine-tuning enables privacy-preserving LLM adaptation but faces a critical bottleneck: the disparity between LLMs' high memory demands and edge devices' limited capacity. To break the memory barrier, we propose Chain Federated Fine-Tuning (ChainFed), an innovative paradigm that forgoes end-to-end updates in favor of a sequential, layer-by-layer manner. It first trains the initial adapter to convergence, freezes its weights, and then proceeds to the next. This iterative train-and-freeze process forms an optimization chain, gradually enhancing the model's task-specific proficiency. ChainFed further integrates three core techniques: 1) Dynamic Layer Co-Tuning to bridge semantic gaps between sequentially tuned layers and facilitate information flow; 2) Globally Perceptive Optimization to endow each adapter with foresight beyond its local objective; 3) Function-Oriented Adaptive Tuning to automatically identify the optimal fine-tuning starting point. Extensive experiments on multiple benchmarks demonstrate the superiority of ChainFed over existing methods, boosting average accuracy by up to 46.46\%.

==> Table/table1_overall_performance.tex <==
\definecolor{steelbluev2}{HTML}{DAE8FC}
\definecolor{steelblue}{HTML}{82B0D2}
\begin{table*}[t]
\footnotesize % 将字体设置为更小的大小
\renewcommand{\arraystretch}{0.98} 
\setlength{\tabcolsep}{9pt} % 调整列间距

  \centering
  % \resizebox{0.94\textwidth}{!}{ % 保持表格自适应宽度
  
    \begin{tabular}{lccccccccc}
    \toprule[1pt]
    \multirow{2}{*}{\textbf{Method}} &  \multicolumn{2}{c}{\textbf{YELP-P}} & \multicolumn{2}{c}{\textbf{AGNEWS}}  & \multicolumn{2}{c}{\textbf{YAHOO}} & \multicolumn{2}{c}{\textbf{20NEWS}} & \multirow{2}{*}{\textbf{Average}}  \\
    \cmidrule(lr){2-3}
    \cmidrule(lr){4-5}
    \cmidrule(lr){6-7}
    \cmidrule(lr){8-9}

    & \textbf{IID} & \textbf{Non-IID}& \textbf{IID} & \textbf{Non-IID}& \textbf{IID} & \textbf{Non-IID}& \textbf{IID} & \textbf{Non-IID}&  \\
    \midrule

    \textbf{Sequence Length}             & \textbf{256} & \textbf{256} & \textbf{64} & \textbf{64} & \textbf{256} & \textbf{256} & \textbf{256} & \textbf{256} & \textbf{$/$} \\
    \midrule[1pt]

    \multicolumn{10}{c}{\textbf{DistilBERT-base}} \\ % 3表示跨越3列，居中对齐
    \midrule[1pt]
    Linear Probing~\cite{kornblith2019better} & 71.56 & 67.53 & 85.76 & 82.84 & 59.22 & 57.13 & 73.74 & 69.83  &70.95 \textcolor{orange}{($\downarrow$ 11.49)}\\ 
    FedAdapter~\cite{cai2022fedadapter}                  
                            & 82.16 & 78.57 & 89.00 & 84.41 & 68.07 & 64.82 & 76.29 & 72.89 &77.03 \textcolor{orange}{($\downarrow$ 5.41)} \\ 
    FwdLLM~\cite{xu2023fwdllm}                      
                            & 82.00 & 77.61 & 88.79 & 83.03 & 65.77 & 61.93 & 63.70 & 59.34 &72.77 \textcolor{orange}{($\downarrow$ 9.67)} \\ 
    FedRA~\cite{su2024fedra}                       
                            & 81.55 & 77.91 & 88.92 & 84.25 & 68.36 & 65.03 & 76.66 & 72.71 &76.92  \textcolor{orange}{($\downarrow$ 5.52)} \\
    C2A~\cite{kim2023client}                       
                            & 80.24 & 76.95 & 87.49 & 82.88 & 66.24 & 61.87 & 74.65 & 70.47 &75.10 \textcolor{orange}{($\downarrow$ 7.34)} \\ 
    % \rowcolor{cyan!10}
    \textbf{\textit{Profit-2-0.8}}     \cellcolor{cyan!10}
      & \underline{85.08}    \cellcolor{cyan!10}
      & \underline{82.89}     \cellcolor{cyan!10}
      & \underline{91.29}     \cellcolor{cyan!10}
      & \underline{88.05}     \cellcolor{cyan!10}
      & \underline{72.54}     \cellcolor{cyan!10}
      & \underline{69.18}     \cellcolor{cyan!10}
      & \underline{80.99}     \cellcolor{cyan!10}
      & \underline{76.24}     \cellcolor{cyan!10}
      & \underline{80.78}     \cellcolor{cyan!10}
      \textcolor{orange}{($\downarrow$ 1.66)}  \\ 
    \rowcolor{cyan!10}
    \textbf{\textit{Profit-3-0.8}}       & \textbf{86.53} & \textbf{84.13} & \textbf{92.59} & \textbf{90.25} & \textbf{73.70} & \textbf{70.41} & \textbf{82.37} & \textbf{79.57} & \textbf{82.44}   \\
    \midrule
    \rowcolor{my_yellow!30}
    Full Fine-tuning$^{\dagger}$\cite{kim2023client} & 87.39 & 85.05 & 93.41 & 91.13 & 75.65 & 73.35 & 84.76 & 82.81 & 84.19  \textcolor{green!50!black}{($\uparrow$ 1.75)}\\

    \midrule[1pt]
    \multicolumn{10}{c}{\textbf{BERT-base}} \\ % 3表示跨越3列，居中对齐
    \midrule[1pt]
    Linear Probing~\cite{kornblith2019better}  & 69.09 & 64.96 & 79.88 & 71.55 & 55.23 & 52.82 & 67.62 & 60.97 & 65.27 \textcolor{orange}{($\downarrow$ 16.85)} \\ 
    FedAdapter~\cite{cai2022fedadapter}                  & 77.84 & 72.59 & 88.41 & 84.03 & 62.67 & 59.74 & 69.42 & 65.76 & 72.56 \textcolor{orange}{($\downarrow$ 9.56)} \\ 
    FwdLLM~\cite{xu2023fwdllm}                      & 81.86 & 77.38 & 87.47 & 80.68 & 66.05 & 62.16 & 5.21$^*$ & 5.01$^*$ &  58.23 \textcolor{orange}{($\downarrow$ 23.89)} \\ 
    FedRA~\cite{su2024fedra}                       & 82.26 & 78.67 & 88.04 & 83.07 & 68.97 & 65.58 & 77.45 & 73.47 & 77.19 \textcolor{orange}{($\downarrow$ 4.93)} \\
    C2A~\cite{kim2023client}                         & 76.39 & 71.16 & 86.81 & 82.11 & 60.78 & 55.73 &68.14  & 61.92  & 70.38 \textcolor{orange}{($\downarrow$ 11.74)}\\
    \rowcolor{cyan!10}
    \textbf{\textit{Profit-3-0.9}}       & \underline{84.46} &  \underline{82.68} &  \underline{91.05} &  \underline{89.11} &  \underline{71.51} &  \underline{67.96} & \underline{79.92}  & \underline{75.13}  &  \underline{80.22}  \textcolor{orange}{($\downarrow$ 1.90)} \\

    \rowcolor{cyan!10}
    \textbf{\textit{Profit-4-0.9}} & \textbf{86.40} & \textbf{84.05} & \textbf{91.89} & \textbf{89.67} & \textbf{73.65} & \textbf{70.17} & \textbf{82.21} & \textbf{78.94} &\textbf{82.12} \\ 
    \midrule
    \rowcolor{my_yellow!30}
    Full Fine-tuning$^{\dagger}$\cite{kim2023client} & 88.15 & 85.92 & 93.82 & 91.53 & 75.84 & 73.68 & 85.72 & 83.09  &84.72  \textcolor{green!50!black}{($\uparrow$ 2.60)}\\ 

    \midrule[1pt]
    \multicolumn{10}{c}{\textbf{RoBERTa-large}} \\ % 3表示跨越3列，居中对齐
    \midrule[1pt]
    Linear Probing~\cite{kornblith2019better} & 66.45 & 62.24 & 69.88 & 62.67 & 50.35 & 48.03 & 60.93 & 51.64 &59.02 \textcolor{orange}{($\downarrow$ 23.72)} \\
    FedAdapter~\cite{cai2022fedadapter}                  & --- & --- & 78.59 & 73.87 & --- & --- & --- & --- &---  \\ 
    FwdLLM~\cite{xu2023fwdllm}  & 76.89 & 72.46 & 80.41 & 74.52 & 58.97 & 55.24 & 5.13$^*$ & 5.05$^*$ & 53.58 \textcolor{orange}{($\downarrow$ 29.16)} \\
    FedRA~\cite{su2024fedra}                       & 77.45 & 73.71  &  81.56 & 76.63  & 61.69 & 58.37 & 69.27 & 65.31&70.50 \textcolor{orange}{($\downarrow$ 12.24)}\\
    C2A~\cite{kim2023client}                         & --- & --- &  76.93 & 71.98  & --- & --- & --- & --- &--- \\ 

    \rowcolor{cyan!10}
    \textbf{\textit{Profit-4-0.8}}       & \underline{86.47} & \underline{83.08} & \underline{91.96} & \underline{89.52} & \underline{72.77} & \underline{69.24} & \underline{81.12} & \underline{76.32} &\underline{81.31} \textcolor{orange}{($\downarrow$ 1.43)} \\

    \rowcolor{cyan!10}
    \textbf{\textit{Profit-5-0.8}}       &\textbf{87.08} & \textbf{84.59} & \textbf{92.93} & \textbf{90.61} & \textbf{73.87} & \textbf{70.60} & \textbf{82.51} & \textbf{79.70} &\textbf{82.74}  \\
    \midrule
    \rowcolor{my_yellow!30}
    Full Fine-tuning$^{\dagger}$\cite{kim2023client} & 88.83 & 86.76 & 93.95 & 91.67 & 76.22 & 74.03 & 86.64 & 83.52 &85.20 \textcolor{green!50!black}{($\uparrow$ 2.46)}\\ 
    \bottomrule[1pt]
    \end{tabular}%
  
  \vspace{-1mm}
  \caption{\textbf{Performance comparison of \textbf{\textit{Profit}} and baselines.} \textbf{Bold} indicates the optimal results, while \underline{underlined} represents the sub-optimal results. \textbf{\textit{Profit-Q-T}} represents the configuration where $Q$ denotes the number of adapters co-trained in each stage, and $T$ specifies the threshold for determining the optimal fine-tuning starting point. The $-$ symbol indicates that the corresponding algorithm fails to function under this setup due to memory constraints, while * denotes that the algorithm cannot converge in this setting.}
\label{tab_overall_performance}
  \vspace{-5mm}
\end{table*}

